Enabling Low-Cost Secure Computing on Untrusted In-Memory Architectures

Modern computing systems are limited in performance by the memory bandwidth available to processors, a problem known as the memory wall. Processing-in-Memory (PIM) promises to substantially improve this problem by moving processing closer to the data, improving effective data bandwidth, and leading to superior performance on memory-intensive workloads. However, integrating PIM modules within a secure computing system raises an interesting challenge: unencrypted data has to move off-chip to the PIM, exposing the data to attackers and breaking assumptions on Trusted Computing Bases (TCBs). To tackle this challenge, this paper leverages multi-party computation (MPC) techniques, specifically arithmetic secret sharing and Yao's garbled circuits, to outsource bandwidth-intensive computation securely to PIM. Additionally, we leverage precomputation optimization to prevent the CPU's portion of the MPC from becoming a bottleneck. We evaluate our approach using the UPMEM PIM system over various applications such as Deep Learning Recommendation Model inference and Logistic Regression. Our evaluations demonstrate up to a $14.66\times$ speedup compared to a secure CPU configuration while maintaining data confidentiality and integrity when outsourcing linear and/or nonlinear computation.

==> Figures/usenix-security-25-ae-latex/usenix25-ae.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Artifact Appendix Template for Usenix Security'25 AE


\appendix
\section{Artifact Appendix}
% \textit{This artifact appendix is meant to be a self-contained document which
% describes a roadmap for the evaluation of your artifact. It should include a
% clear description of the hardware, software, and configuration requirements. In
% case your artifact aims to receive the functional or results reproduced badge,
% it should also include the major claims made by your paper and instructions on
% how to reproduce each claim through your artifact. Linking the claims of your
% paper to the artifact is a necessary step that ultimately allows artifact
% evaluators to reproduce your results.}

% \textit{Please fill all the mandatory sections, keeping their titles and
% organization but removing the current illustrative content, and remove the
% optional sections where those do not apply to your artifact.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
Our artifact contains all necessary source codes and scripts for evaluating our proposed security scheme.
This paper leverages Multi-Party Computation (MPC) techniques, specifically arithmetic secret sharing, and Yao's garbled circuits, to securely outsource bandwidth-intensive computation to PIM. Additionally, we employ precomputation optimizations to prevent the CPU's portion of the MPC from becoming a bottleneck. 
We provided all the source codes and scripts for evaluating our scheme using UPMEM, the first publicly available PIM, over four data-intensive applications: Multilayer Perceptron inference (MLP), Deep Learning Recommendation Model inference (DLRM), linear regression training, and logistic regression training. 
This artifact allows researchers to reproduce our results, explore this area further, and expand our work. With this artifact, researchers can regenerate the performance results for UPMEM-Precompute-C(V), UPMEM-Runtime-C(V), and UPMEM-Runtime-A(2Y)-C(V), as presented in figures 13 to 18.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description \& Requirements}

% \textit{[Mandatory] This section should list all the information necessary to
% recreate the same experimental setup you have used to run your artifact. Where
% it applies, the minimal hardware and software requirements to run your artifact.
% It is also very good practice to list and describe in this section benchmarks
% where those are part of, or simply have been used to produce results with, your
% artifact.}

\subsubsection{Security, privacy, and ethical concerns}
% \textit{[Mandatory] Describe any risk for evaluators while executing your
% artifact to their machines security, data privacy or others ethical concerns.
% This is particularly important if destructive steps are taken or security
% mechanisms are disabled during the execution.}
Our research does not compromise user privacy or safety, and all data used in our experiments is either synthetic or randomly generated. Therefore, no Personally Identifiable Information (PII), sensitive data, or human subjects were involved.

\subsubsection{How to access}
% {\em [Mandatory]} \textit{Describe here how to access your artifact. If you are
% applying for the Artifacts Available badge, the archived copy of the artifacts
% must be accessible via a stable reference or DOI. For this purpose, we recommend
% Zenodo, but other valid hosting options include institutional and
% third-party digital repositories (e.g., FigShare, Dryad, Software
% Heritage, GitHub, or GitLab — not personal webpages). For repositories that can
% evolve over time (e.g., GitHub), a stable reference to the evaluated version
% (e.g., a URL pointing to a commit hash or tag) rather than the evolving version
% reference (e.g., a URL pointing to a mere repository) is required. Note that the
% stable reference provided at submission time is for the purpose of Artifact
% Evaluation. Since the artifact can potentially evolve during the evaluation to
% address feedback from the reviewers, another (potentially different) stable
% reference will be later collected for the final version of the artifact (to be
% included here for the camera-ready version).}
The code is open-source and hosted on a GitHub public repository to facilitate reuse. Additionally, it is archived on Zenodo. We encourage other researchers to explore, reproduce, and modify our code, provided they give appropriate credit.
\begin{itemize}[nosep]
    \item GitHub: \href{https://github.com/Secure-UPMEM/SecUPMEM.git}{github.com/Secure-UPMEM/SecUPMEM.git}.

    \item Zenodo: \href{https://zenodo.org/records/14869014}{zenodo.org/records/14869014}.
\end{itemize}

\subsubsection{Hardware dependencies}
% {\em [Mandatory]} \textit{Describe any specific hardware features required to
% evaluate your artifact (vendor, CPU/GPU/FPGA, number of processors/cores,
% microarchitecture, interconnect, memory, hardware counters, etc). If your
% artifact requires special hardware, please provide instructions on how to gain
% access to the hardware. For example, provide private SSH keys to access the
% machines remotely. Please keep in mind that the anonymity of the reviewers needs
% to be maintained and you may not collect or request personally identifying
% information (e.g., email, name, address). [Simply write "None." where this does
% not apply to your artifact.]}
To evaluate our method, we utilize UPMEM PIM hardware, which primarily consists of standard DDR4-2400 DIMMs integrated with DPUs. Our setup includes 20 PIM-enabled DIMMs, providing a total of 160GB of MRAM and 2560 DPUs working in parallel at a clock frequency of 350 MHz. The host server for the UPMEM system is equipped with a 2-socket Intel Xeon Silver 4110 CPU. To accurately reproduce our results, access to the actual hardware is necessary. UPMEM’s PIM data centers are accessible upon request at \url{https://www.upmem.com/developer.}

\subsubsection{Software dependencies}\label{software}
% {\em [Mandatory]} \textit{Describe any specific OS and software packages
% required to evaluate your artifact. This is particularly important if you share
% your source code and it must be compiled or if you rely on some proprietary
% software that you cannot include in your package. In such a case, you must
% describe how to obtain and to install all third-party software, data sets, and
% models. [Simply write "None." where this does not apply to your artifact.]}
All the implemented applications require the UPMEM SDK, which can be installed based on the hardware specifications and is accessible at \url{https://sdk.upmem.com.} 
For dependencies related to MLP, DLRM, logistic regression, and linear regression, please refer to our baseline implementations as our work is built upon them.
\begin{itemize}[nosep]
    \item MLP \href{https://github.com/CMU-SAFARI/prim-benchmarks} {(Link)}
    \item DLRM \href{https://github.com/UBC-ECE-Sasha/PIM-Embedding-Lookup}{ (Link 1,}
    \href{https://github.com/upmem/PIM-Embedding-Lookup/tree/multicol/upmem}{ Link 2)} 
    \item Logistic and Linear Regression \href{https://github.com/CMU-SAFARI/pim-ml}{ (Link 1,} \href{https://github.com/CMU-SAFARI/prim-benchmarks}{ Link 2)} 
\end{itemize}
\vspace{3mm}

\subsubsection{Benchmarks}
% {\em [Mandatory]} \textit{Describe here any data (e.g., data-sets, models,
% workloads, etc.) required by the experiments with this artifact reported in your
% paper.} \textit{[Simply write "None." where this does not apply to your
% artifact.]}

Our scheme is evaluated using MLP inference, DLRM inference, logistic regression training, and linear regression training.
To evaluate our implementation, we use randomly generated inputs.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Set-up}
% {\em [Mandatory]} \textit{This section should include all the installation and
% configuration steps required to prepare the environment to be used for the
% evaluation of your artifact.}

\subsubsection{Installation}
% {\em [Mandatory]} \textit{Instructions to download and install dependencies as
% well as the main artifact. After these steps the evaluator should be able to run
% a simple functionality test.}
To run this artifact on your local device, the UPMEM SDK must first be installed, which is available at \url{https://sdk.upmem.com}. However, as previously mentioned, reproducing our results requires access to real hardware (20 UPMEM PIMs) rather than the simulator.
Once the UPMEM SDK is installed, the artifact can be downloaded from \href{https://github.com/Secure-UPMEM/SecUPMEM.git}{GitHub} and \href{https://zenodo.org/records/14736864}{Zenodo}.

% If you are hoping to use your own system to run our code, you need to install the UPMEM SDK first, which is accessible at \url{https://sdk.upmem.com}. However, as previously mentioned, reproducing our results requires access to real hardware rather than the simulator.
% After installing the UPMEM SDK, you can download our artifact from \href{https://github.com/Secure-UPMEM/SecUPMEM.git}{GitHub} and \href{https://zenodo.org/records/14736864}{Zenodo}.

\subsubsection{Basic Test}
% {\em [Mandatory]} \textit{Instructions to run a simple functionality test. Does
% not need to run the entire system, but should check that all required software
% components are used and functioning fine. Please include the expected successful
% output and any required input parameters.}
% To run a simple functionality check, you can run "./run\_functionality.sh" in the root folder which will run a simple test on all the applications and you will expect all the applications to run one after the other and output execution time. If you wish to only run one of the applications, you can redirect to the the folder associated with the specific application and then run "run\_functionality.sh.

Script \textit{run\_functionality.sh}, in the root directory, can be used to perform a simple functionality check. This file executes a basic test on all the applications sequentially and outputs execution time. To run a specific application, the \textit{run\_functionality.sh} script in the corresponding folder can be executed.

% To perform a simple functionality check, use  \textit{run\_functionality.sh} script in the root folder, which executes a basic test on all applications. This script sequentially runs all applications and outputs their execution times.
% To run a specific application, navigate to its corresponding folder and execute \textit{run\_functionality.sh}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace
\subsection{Evaluation workflow}
% {\em [Mandatory for Artifacts Functional \& Results Reproduced, optional for
% Artifact Available]} \textit{This section should include all the operational
% steps and experiments which must be performed to evaluate if your your artifact is
% functional and to validate your paper's key results and claims. For that
% purpose, we ask you to use the two following subsections and cross-reference the
% items therein as explained next.}

\subsubsection{Major Claims}
% {\em [Mandatory for Artifacts Functional \& Results Reproduced, optional for
% Artifact Available]} \textit{Enumerate here the major claims (Cx) made in your
% paper. Follows an example:}\\
Our major claim is as follows:

\begin{compactdesc}

    % \item[(C1):] \textit{System\_name achieves the same accuracy of the state-of-the-art
    % systems for a task X while saving 2x storage resources. This is proven by
    % the experiment (E1) described in [refer to your paper's sections] whose
    % results are illustrated/reported in [refer to your paper's plots, tables,
    % sections or the sort].}

    % \item[(C2):] \textit{System\_name has been used to uncover new bugs in the Y
    % software. This is proven by the experiments (E2) and (E3) in [ibid].}
    \item[(C1):] 
Compared to a secure CPU implementation, our framework achieves speedups of $14.66\times$, $9.80\times$, $2.64\times$, and $5.85\times$ for MLP inference, DLRM inference, Linear Regression training, and Logistic Regression training, respectively. This is proven by the experiment (E1) described in Section 7.1 whose results are illustrated in Figures 14, 15, 16, 18.

\end{compactdesc}

\subsubsection{Experiments}
% {\em [Mandatory for Artifacts Functional \& Results Reproduced, optional for
% Artifact Available]} \textit{Link explicitly the description of your experiments
% to the items you have provided in the previous subsection about Major Claims.
% Please provide your estimates of human- and compute-time for each of the listed
% experiments (using the suggested hardware/software configuration above). Follows
% an example:}

% use paralist for more compact list format: for more details check here:
% https://texfaq.org/FAQ-complist
\begin{compactdesc}

    % \item[(E1):] \textit{[Optional Name] [30 human-minutes + 1 compute-hour + 5GB disk]:
    % provide a short explanation of the experiment and expected results.}

    % \begin{asparadesc}
    %     \item[How to:]  \textit{Describe thoroughly the steps to perform the
    %     experiment and to collect and organize the results as expected from your
    %     paper. We encourage you to use the following structure with three main
    %     blocks for the description of your experiment.}

    %     \item[Preparation:] \textit{Describe in this block the steps required to
    %     prepare and configure the environment for this experiment.}

    %     \item[Execution:]
    %     \textit{Describe in this block the steps to run this experiment.}

    %     \item[Results:] \textit{Describe in this block the steps required to
    %     collect and interpret the results for this experiment.}
    % \end{asparadesc}

    % \item[(E2):] \textit{[Optional Name] [1 human-hour + 3 compute-hour]: ...}

    % \item[(E3):] \textit{[Optional Name] [1 human-hour + 3 compute-hour]: ...}
 \item[(E1):]
 [30 human-minutes + 2.5 compute-hour + 32GB disk]:

    \begin{asparadesc}
        \item[How to:] Our results can be reproduced by following the three steps below.

        \item[Preparation:] 
        % If you have access to UPMEM servers, you just need to clone our GitHub repository to run the code. If you want to prepare your own system, first you need to install UPMEM SDK as mentioned in section \ref{software}. Then, you need to clone our repository.  
Install the UPMEM SDK, as described in Section \ref{software}, then clone our artifact.
        
        % If you have access to UPMEM servers, simply clone our GitHub repository to run the code. If you are setting up your own system, you must first install the UPMEM SDK, as described in section \ref{software}, before cloning our repository.  


        \item[Execution:]
        Script \textit{./run\_reproduce.sh}, in the root directory, can be used to regenerate our results. This file executes all the applications with our configuration sequentially and outputs execution time for UPMEM-Precompute-C(V), UPMEM-Runtime-C(V), and UPMEM-Runtime-A(2Y)-C(V), as presented in Figures 13 to 18. To reproduce the results for a specific application, the \textit{./run\_reproduce.sh} script in the corresponding folder can be executed.
        
        % To reproduce our results, use the \textit{./run\_reproduce.sh} script in the root folder, which runs all four applications with our configurations. This script sequentially runs all applications and outputs their execution times.
        % To run a specific application, navigate to its corresponding folder and execute \textit{./run\_reproduce.sh}.

        This script compiles and links the host and DPU source codes for a specific number of DPUs and tasklets. There is a Makefile for each application that facilitates the compilation and linking of the source codes.  
        
        % To reproduce our results, you can run "./run\_reproduce.sh" in the root folder, which will run all four applications with the same configuration as our experiments. You should expect all the applications to run one after the other and output execution times. If you wish to run only one of the applications, you can redirect to the folder associated with the specific application and then run "run\_reproduce.sh. If you do not want to use our scripts, you need to compile and link the host and DPU source codes. During the compilation stage, you must specify the number of DPUs and the number of tasklets. Similar to our baseline configurations, there is a Makefile for each application that facilitates the compilation and linking of the source codes. 
        
        \item[Results:]  After running our script, the final execution time is reported. Table \ref{tab:notations} explains the different notations used for manually determining execution times. The execution time is calculated using the formula provided below:    
        % After running our script, the final execution time is reported. Table \ref{tab:notations} explains the timings you will encounter for manually finding the execution times. This execution time is calculated using the formula provided below:
    % \vspace{-2mm}    
\[
PIM\ Time = CPU-DPU + PIM\ kernel + DPU-CPU
\]
% \vspace{-3mm}  
\[
Kernel\ time = Max[CPU\ Time, PIM\ Time]
\]
% \vspace{-3mm}  
\[
Execution\ time = Kernel\ time + Merge + Verification
\]


\begin{table}[htp]
	\centering
	\caption{List of timing notations}
	\scalebox{0.80}{
	\begin{tabular}{>{\centering\arraybackslash}p{1in}>{\centering\arraybackslash}p{2.5in}}
		\toprule
  Timing notations & Explanation\\
		\midrule
    $CPU-DPU$& CPU to DPUs transfer time \vspace{1mm}\\
    $DPU-CPU$ & DPUs to CPU transfer time \vspace{1mm}\\
    $ PIM\ kernel$& Kernel execution time on DPUs \vspace{1mm}\\
     $CPU\ Time$ & Kernel execution time on CPU \vspace{1mm}\\
     $Kernel\ time$ & The maximum of CPU Time and PIM Time \vspace{1mm}\\
     $Merge$ & Merging time of CPU and PIM results \vspace{1mm}\\
     $Verification$ & Verification time \vspace{1mm}\\
		\bottomrule
	\end{tabular}}
	\label{tab:notations}
 \vspace{0.2cm}
% \vspace{-1em}
\end{table}
    \end{asparadesc}
\end{compactdesc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Notes on Reusability}
% \label{sec:reuse}
% {\em [Optional]} \textit{This section is meant to optionally share additional
% information on how to use your artifact beyond the research presented in your
% paper. In fact, a broader objective of an artifact evaluation is to help you
% make your research reusable by others.}

% \textit{You can include in this section any sort of instruction that you believe
% would help others re-use your artifact, like, for example, scaling down/up
% certain components of your artifact, working on different kinds of input or
% data-set, customizing the behavior replacing a specific module/algorithm, etc.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Version}
%%%%%%%%%%%%%%%%%%%%
% Obligatory.
% Do not change/remove.
%%%%%%%%%%%%%%%%%%%%
Based on the LaTeX template for Artifact Evaluation V20231005. Submission,
reviewing and badging methodology followed for the evaluation of this artifact
can be found at \url{https://secartifacts.github.io/usenixsec2025/}.
